Towards Usable Parental Control for Voice Assistants

Voice Personal Assistants (VPA) have become a common household appliance. As one of the leading platforms for VPA technology, Amazon created Alexa and designed Amazon Kids for children to safely enjoy the rich functionalities of VPA and for parents to monitor their kids' activities through the Parent Dashboard. Although this ecosystem is in place, the usage of Parent Dashboard is not yet popularized among parents. In this paper, we conduct a parent survey to find out what they like and dislike about the current parental control features. We find that parents need more visuals about their children's activity, easier access to security features for their children, and a better user interface. Based on the insights from our survey, we present a new design for the Parent Dashboard considering the parents' expectations.

==> evaluation.tex <==
\section{Evaluation}
In our survey, we showed participants 3 security features, and asked them how effective they think these features are. We further investigated if participants preferred a specific security feature and think it's more effective. First, we selected participants who rated the effectiveness of all three security features (participants who answered questions E2, F2 and G3 of the survey, see appendix), and got 14 qualified responses. Next, we encoded text responses from extremely ineffective - extremely effective to 1 - 5 for further calculation. Finally, we turned the collected data into a 3 $\times$ 1 within-subject experiment, where the dependent variable is participants' rating of effectiveness. Table \ref{tab:anova-table} shows the ANOVA table, which indicated that The effect of f1 (security feature) on the dv (rating of effectiveness) was not statistically significant $(F(2, 26) = 1.696, p > 0.05)$. This might be due to the limited number of qualified responses. 
\begin{table}[H]
\centering
\begin{tabular}{cccccc}
\hline
\textit{Effect} & df & SS     & MS    & F     & P      \\ \hline
Participant     & 13 & 16.119 & 1.240 &       &        \\
F1              & 2  & 1.000  & 0.500 & 1.696 & 0.2031 \\
F1\_x\_Par      & 26 & 7.667  & 0.295 &       &        \\ \hline
\end{tabular}
\\
\caption{ANOVA Table for Security Features}
\label{tab:anova-table}
\end{table}
